Full LTL Synthesis over Infinite-state Arenas

Recently, interest has increased in applying reactive synthesis to richer-than-Boolean domains. A major (undecidable) challenge in this area is to establish when certain repeating behaviour terminates in a desired state when the number of steps is unbounded. Existing approaches struggle with this problem, or can handle at most deterministic games with B\"uchi goals. This work goes beyond by contributing the first effectual approach to synthesis with full LTL objectives, based on Boolean abstractions that encode both safety and liveness properties of the underlying infinite arena. We take a CEGAR approach: attempting synthesis on the Boolean abstraction, checking spuriousness of abstract counterstrategies through invariant checking, and refining the abstraction based on counterexamples. We reduce the complexity, when restricted to predicates, of abstracting and synthesising by an exponential through an efficient binary encoding. This also allows us to eagerly identify useful fairness properties. Our discrete synthesis tool outperforms the state-of-the-art on linear integer arithmetic (LIA) benchmarks from literature, solving almost double as many syntesis problems as the current state-of-the-art. It also solves slightly more problems than the second-best realisability checker, in one-third of the time. We also introduce benchmarks with richer objectives that other approaches cannot handle, and evaluate our tool on them.

==> acceleration.tex <==
\subsection{Acceleration}

The approach described above attempts synthesis through a classic lazy CEGAR loop adapted substantially for synthesis. However, as with all CEGAR approaches for infinite-state problems, there is a risk that the approach will explore the wrong part of the state space, and end up not terminating. 
As an alternative, we also contribute a more eager procedure that identifies liveness properties of the program by syntactically inspecting the problem. 
The evaluation shows this is often enough to solve the synthesis problem; if not, the CEGAR approach is applied starting from this more precise abstraction.

We do this by identifying terms in the problem from which well-founded relations can be constructed.
For instance, the relation $v_{prev} > v$ (that captures when $v$ decreases) is not well-founded when $v$ is an integer, but it is when $v$ is a natural, that is, w.r.t. the invariant
$0 \leq v$.
Indeed, there is no infinite execution where $0 \leq v$ remains true and $v$ decreases infinitely often. We call $v$ a ranking function when the relation $v_{prev} > v$ is well-founded modulo some invariant.

\begin{definition}[Ranking functions]
    A function $r : \Val(V) \rightarrow R$, for a range $R$, is said to be a \emph{ranking function} modulo an \emph{invariant} $inv$ in a arena $\arena$ iff for every execution $w \in L(P)$ $w$ has no suffix $w'$ such that in $w'$ the invariant is always true and $r$ decreases infinitely often, with only a finite amount of increases.
\end{definition}

We extract ranking functions from predicates that appear syntactically in the problem. We normalise such a predicate $p \mydef x \leq y$, to $0 \leq y - x$. Then, if $y$ and $x$ are both integer variables, we are assured that $y - x$ is a ranking function w.r.t. the invariant $p$. 
This does not hold for real number variables. Instead, an analysis of whether updates of the variables can decrement with successively smaller values, is needed to determine well-foundedness. Our tool targets discrete problems, for which LIA suffices, thus we do not discuss this further.

Then to refine an abstraction with information about a term's well-foundedness, it is sound to require that if a run features infinitely many decreases then it also has infinitely many increases or violations of the invariant.

\begin{definition}[Ranking Abstraction]
    For a ranking function $r$ w.r.t. an invariant $inv$, let $r^{dec} = r_{prev} > r$ and $r^{inc} = r_{prev} < r$, then we define the ranking abstraction $\alpha_{rk}(P, r) \mydef GF(r^{dec}) \implies GF(r^{inc} \vee \neg inv)$.
\end{definition}

This approach can be used also for loops exposed by a counterexample:
if we discover a ranking function that proves termination, we can use it in a general way as a well-founded term.
This would be applicable to the entire state-space rather than a particular loop. 
However, sophisticated ranking functions (e.g., lexicographic ranking functions) could incur an overhead in terms of added predicates, so we use structural loop refinement as default. 
Acceleration gives an abstraction that
contains all predicates in the problem and the derived ranking abstractions,
which can be a valuable starting point, as
our evaluation will show.










\begin{toappendix}
\begin{propositionrep}[Ranking Abstraction Correctness]
    Given a ranking function $r$ with invariant $inv$, then $\alpha(\arena, Pr \cup \{r^{dec}, r^{inc}, inv\}) \wedge \alpha_{rk}(\arena, r)$ is an abstraction of $\arena$. 
\end{propositionrep}
\begin{proof}
    $\alpha(\arena, Pr)$ is an abstraction of $\arena$, and thus also $\alpha(\arena, Pr \cup \{r^{dec}, r^{inc}, inv\})$. What is left to show is that $\alpha_{rk}(\arena, r)$ also is an abstraction of $\arena$. Note, every abstract trace in $L(\alpha_{rk}(\arena, r))$ satisfies that either eventually always $r$ does not decrease, or infinitely often it both decreases, and increases or violates the invariant. Consider a concrete word, by the property of $r$ being a ranking function modulo $\arena$, every concrete word will exhibit exactly this behaviour, and thus the corresponding abstract word will be in $L(\alpha_{rk}(\arena, r))$. \qed
\end{proof}
    
\end{toappendix}







\begin{toappendix}
Here we prove that applying ranking refinement instead of structural loop refinement ensures progress.

\begin{propositionrep}[Ranking Refinement Progress]
    For abstraction $\alpha(P, Pr)$ allowing a \counterstrategy $\moore$ with a finite counterexample $ce$ that induces a lasso in $\moore$ and a ranking function $r$, then abstraction $\alpha(P, Pr \cup \{r_{dec}, r_{inc}\}) \wedge \alpha_{rk}(P, r)$ does not allow counterexamples that induce the same refinement.
\end{propositionrep}
\begin{proof}
    
    Suppose that the abstraction $\alpha(A, Pr \cup \{r_{dec}, r_{inc}\}) \wedge \alpha_{rk}(A, r)$ contains a word $a$ unconcretisable w.r.t. $\arena$, with a prefix $a_0,\ldots, a_l,\ldots, a_k$, such that concretisability fails only on $a_k$, $a_k = a_l$, and the suffix of the word is of the form $(a_l,\ldots, a_k-1)^\omega$.\footnote{This is an equivalent condition to finding a lasso in a \counterstrategy.}
    
    If concretisability fails because of a transition predicate mismatch then a ranking refinement is not applicable, thus the result holds.

    Consider that concretisability fails because of a state predicate mismatch, and thus ranking refinement is applicable. Consider also that $a$ induces the same ranking function $r$. Thus $r$ is strictly decreasing in the transitions corresponding to $(a_l,\ldots, a_k-1)^\omega$. Given $\alpha_{rk}(\arena, r)$, $r_{inc}$ must not be guessed as true in any of $a_l,\ldots, a_k-1$, otherwise given $r$ is a ranking function for this loop, the concretisability would have failed earlier than $a_k$ on the wrong guess of $r_{inc}$. Similarly if $r_{dec}$ is guessed as false throughout. Then only $r_{dec}$ is guessed as true in $a_l,\ldots, a_k-1$, giving a contradiction, since then the word is not in $\alpha_{rk}(P, r)$. \qed
    
\end{proof}
    
\end{toappendix}




